Online Optimization with Predictions and Non-convex Losses

We study online optimization in a setting where an online learner seeks to optimize a per-round hitting cost, which may be non-convex, while incurring a movement cost when changing actions between rounds. We ask: \textit{under what general conditions is it possible for an online learner to leverage predictions of future cost functions in order to achieve near-optimal costs?} Prior work has provided near-optimal online algorithms for specific combinations of assumptions about hitting and switching costs, but no general results are known. In this work, we give two general sufficient conditions that specify a relationship between the hitting and movement costs which guarantees that a new algorithm, Synchronized Fixed Horizon Control (SFHC), provides a $1+O(1/w)$ competitive ratio, where $w$ is the number of predictions available to the learner. Our conditions do not require the cost functions to be convex, and we also derive competitive ratio results for non-convex hitting and movement costs. Our results provide the first constant, dimension-free competitive ratio for online non-convex optimization with movement costs. Further, we give an example of a natural instance, Convex Body Chasing (CBC), where the sufficient conditions are not satisfied and we can prove that no online algorithm can have a competitive ratio that converges to 1.

==> Figs/Fig_RSFHC_bad_eg.tex <==
\begin{figure}
\begin{center}
\begin{asy}
size(7cm);
pair X1 = (0, 0);
pair X2 = (2, 0);
pair X3 = (4, -8);
pair X4 = (6, 0);
pair X5 = (8, 0);

pair Y1 = (0, -0.5);
pair Y2 = (2, -1);
pair Y3 = (4, -2);
pair Y4 = (6, -1);
pair Y5 = (8, -0.5);

dot(X1, blue+linewidth(5));
label("$v_{t-2}$", X1, N);
dot(X2, blue+linewidth(5));
label("$v_{t-1}$", X2, N);
dot(X3, blue+linewidth(5));
label("$v_{t}$", X3, N);
dot(X4, blue+linewidth(5));
label("$v_{t+1}$", X4, N);
dot(X5, blue+linewidth(5));
label("$v_{t+2}$", X5, N);

dot(Y1, red+linewidth(5));
label("$x_{t-2}^*$", Y1, S);
dot(Y2, red+linewidth(5));
label("$x_{t-1}^*$", Y2, S);
dot(Y3, red+linewidth(5));
label("$x_{t}^*$", Y3, S);
dot(Y4, red+linewidth(5));
label("$x_{t+1}^*$", Y4, S);
dot(Y5, red+linewidth(5));
label("$x_{t+2}^*$", Y5, S);


draw(Y1--Y2, dashed+green);
draw(Y2--Y3, dashed+green);
draw(Y3--Y4, dashed+green);
draw(Y4--Y5, dashed+green);
\end{asy}
\end{center}
\caption{\emph{\textbf{Illustration of the bad "anchor" timestep described in Section \ref{Appendix:Online_Adv}} If the online adversary predicts $t$ is an "anchor" timestep before $f_t$ is revealed, he can manipulate $f_t$ so that $v_t$ is far away from other minimizers but $f_t$ is relative smooth. The online adversary can pick the path $x_{t-2}^*, \cdots, x_{t+2}^*$. However, the online learner will incur a huge movement cost at this timestep because it must pick $x_t = v_t$.}}
\label{figure:RSFHC_bad_eg}
\end{figure}

==> Preliminary.tex <==
We consider online optimization with switching cost over a finite horizon $T$. The switching/movement cost function is $c: \mathbb{R}^d \times \mathbb{R}^d \to \mathbb{R}^+ \cup \{0\}$ and is fixed through timesteps. Now we describe the game setting when the length of the prediction window is $W$. At the beginning of the game, hitting cost functions of the first $W - 1$ timesteps have already been revealed to the online algorithm. At timestep $t \geq 0$, if $t + W \leq T$, the hitting cost function $f_{t+W}$ is revealed to the online algorithm. After observing $f_{t+W}$, the algorithm picks its decision point $x_t \in \mathbb{R}^d$ and incurs both the hitting cost $f_t(x_t)$ and $c(x_t, x_{t-1})$. The total cost incurred by the algorithm is
$$C_T(x) = \sum_{t=1}^T f_t(x_t) + c(x_t, x_{t-1}),$$
where $x = (x_1, x_2, \cdots, x_T)$.

\yiheng{The definition is very similar with \cite{li2018online}. We describe it in a slightly different way in order to introduce the online adversary for the randomized algorithm.}

A commonly suggested algorithm for Smoothed Online Convex Optimization is "receding horizon control" (RHC), which computes the provisioning for the current time by optimizing over a window of predicted future loads (see \cite{lin2012online}). However, it is shown that in the heterogeneous setting considered in \cite{lin2012online}, for any $W \geq 0$, RHC is $\geq (1 + \max_s (\beta_s/e_{0,s}))$-competitive, where $\beta_s$ and $e_{0,s}$ are constants defined by the problem setting. This competitive ratio is bad because it does not tend to $1$ as the length of the prediction window $W$ tends to infinity. In \cite{lin2012online}, a variant of RHC, Averaging Fixed Horizon Control (AFHC), is shown to be $\left(1 + \max_s \frac{\beta_s}{(W + 1)e_{0, s}}\right)$-competitive. \cite{chen2015online} studied the expected competitive ratio, as well as regret and competitive difference, in a more general prediction model where the quality of predictions decreases the further we look into the future. \cite{chen2016using} proceeded on the same general prediction model and proposed an algorithm Committed Horizon Control (CHC). CHC allows arbitrary level of commitments thus subsumes RHC and AFHC. An intuition we summarized from \cite{chen2015online, chen2016using} is that good competitive ratio results are difficult to derive if we adopt the noisy prediction model. For this reason, many later works still concerned with the exact prediction model (See \cite{li2018online, shi2019value}).The authors of \cite{li2018online} studied SOCO with $\ell_2$ squared switching with exact predictions. They proposed the Receding Horizon Gradient Descent (RHGD) and the Receding Horizon Accelerated Gradient (RHAG) frameworks, whose dynamic regrets can achieve an exponential decay rate with respect to the length of the prediction window $W$. By plugging in the Regularized Online Balanced Descent (ROBD) algorithm as the initializer of these frameworks (with a small modification), we immediately achieved an exponential rate for the competitive ratio. \yiheng{Shall we explain this in the appendix?} \cite{shi2019value} proposed a variant of AFHC which can achieve a $1 + \frac{c}{W}$ competitive ratio with small constant $c$ in some specific problem settings.

\begin{definition}[Use prediction efficiently]\label{def:efficient_pred}
We say a SOCO algorithm $ALG$ for a problem setting $P$ can leverage the prediction window efficiently if there exists a function $g: \mathbb{R}^+ \to \mathbb{R}^+$ which is independent with the number of total timesteps $T$, such that $\forall \epsilon > 0$, $\forall W \geq g(\epsilon)$, $ALG$ with a prediction window of length $W$ has a competitive ratio of at most $(1 + \epsilon)$.
\end{definition}

\yiheng{A new idea is formulating it like this: The problem setting with unknown T is revealed. An algorithm is able to leverage the prediction window efficiently if for any input $\epsilon > 0$, the algorithm can specify a finite $W$ so that its competitive ratio is always upper bound by $1 + \epsilon$ when given a prediction window of length $W$.}

==> Proofs/Proof_quad_CBC_impossible.tex <==
Suppose the game starts from $x_0 = 0$. For $t = 1, \cdots, T - 1$, propose the convex body $K_t = [-1, 1]$. At the last timestep, if the algorithm has picked $x_{T-W} \geq 0$, propose the convex body $K_T = \{-1\}$; else, propose $K_T = \{1\}$. Notice that we can choose $K_T$ based on the algorithm's decision $x_{T - W}$.

Therefore, we obtain that
$$cost(ALG) = \sum_{t=1}^T M_t \geq \sum_{t=T-W+1}^{T}M_t \geq \sum_{t=T-W+1}^{T}\frac{1}{2W^2} = \frac{1}{2W}.$$
However, the offline optimal, with full knowledge of the body sequence, can divide the journey into multiple small steps. Specifically, if $K_T = \{1\}$, the OPT picks $x_t = \frac{t}{T}$; else, the OPT picks $x_t = -\frac{t}{T}$. The total cost of OPT is
$$cost(OPT) = \sum_{t=1}^T M_t^* = \sum_{t=1}^T \frac{1}{2T^2} = \frac{1}{2T}.$$
Therefore, we see that
$$\frac{cost(ALG)}{cost(OPT)} \geq \frac{T}{W}.$$

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)

==> Underlying_problem.tex <==
\subsection{Underlying Online Planning}\label{sec:under}
The game setting considered in Theorem \ref{thm:RRFHC_general_cr_1} present a interesting online planning problem.

Suppose a company is doing investment in some market. Define set $R = \{x_0, x_1, x_2, \cdots\}$ as the set of "good opportunities". If $t \in R$ and the company's investment for this timestep is $c(t)$, it gets a reward of $\eta c(t)$, where $\eta$ is a fixed large coefficient. The game runs as follows:

At timestep $t$, the company guess if time $t + W$ is a "good opportunity" by investing an amount of money $c(t + W)$ to it. Then, if $t \in R$, the company earns $\eta c(t)$, and the market reveals the next "good opportunity" after $t$ to the company.

We assume the market is adversarial when generating the set $R$. However, it has the constraints that $x_0 = 0$ and $x_i < x_{i+1} \leq x_i + W$, which says two consecutive good opportunities cannot be too far away.

The idea of RRFHC translates to a simple randomized algorithm for generating the set $R$: Pick $x_{i+1} = x_i + Y_i$, where $Y_i$ is chosen uniform randomly from the set $\{n \in \mathbb{Z} \mid \frac{W}{2} < n \leq W\}$. The expected total reward received by the company is upper bounded by $\frac{2}{W}\sum_{t = 1}^T c(t)$. The proof sketch is as following:

In the first step, we show that given all the information before timestep $t - W$ (before the company commits $c(t)$), the probability of the event that timestep $t$ is a good opportunity is upper bounded by $\frac{2}{W}$, which is
\begin{equation}\label{Underlying:e0}
    P(t \in R \mid Z_{1:t-W} = z_{1:t-W}) \leq \frac{2}{W}, \forall z_{1:t-W}.
\end{equation}

For convenience, we use $Z_{t_1:t_2}$ (random variables) to denote the information revealed after the company decides $c(t_1 + W - 1)$ at timestep $t_1 - 1$ and before it decides $c(t_2+W)$ at timestep $t_2$. Therefore, we can suppose the cost $c(t+W)$ is determined by some function of the information revealed in the first $t$ rounds, i.e. $c(t+W) = f(z_{1:t})$. In the second step, we bound the expectation of the reward by
\begin{subequations}\label{Underlying:e1}
    \begin{align}
    \mathbb{E}[Reward] ={}& \sum_{t=1}^\infty \sum_{z_{1:t}} P(t \in R \text{ and }Z_{1:t} = z_{1:t})f(z_{1:t-W})\label{Underlying:e1:s1}\\
    ={}& \sum_{t=1}^\infty \sum_{z_{1:t-W}} P(t \in R \mid Z_{1:t-W} = z_{1:t-W})\nonumber\\
    &\cdot P(Z_{1:t-W} = z_{1:t-W})\cdot f(z_{1:t-W})\label{Underlying:e1:s2}\\
    \leq{}& \frac{2}{W} \sum_{t=1}^\infty \sum_{z_{1:t-W}} P(Z_{1:t-W} = z_{1:t-W})f(z_{1:t-W})\label{Underlying:e1:s3}\\
    ={}& \frac{2}{W} \mathbb{E}[Invest].\nonumber
    \end{align}
\end{subequations}
In \eqref{Underlying:e1:s1}, notice that whether $t \in R$ can be determined by the information that $Z_{1:t} = z_{1:t}$. Therefore, for all outcome sequence $z_{1:t}$, we have $P(t \in R \text{ and }Z_{1:t} = z_{1:t}) = P(Z_{1:t} = z_{1:t})$ if $Z_{1:t} = z_{1:t}$ implies $t \in R$, and $P(t \in R \text{ and }Z_{1:t} = z_{1:t}) = 0$ otherwise. In \eqref{Underlying:e1:s2}, we use Bayes Theorem. In \eqref{Underlying:e1:s3}, we use \eqref{Underlying:e0}.

\subsection{A gentle start}
In this section, we aim to solve the dilemma that if a gambler double his stake every round, he can win money for sure. The argument seems to hold even if the coin is biased so that the probability that the gambler wins at every round is $p < 1/2$. The gambler's strategy is doubling his stake every round and leave immediately after he wins. In this way, he can easily promise that $\frac{Reward}{Invest} > \frac{1}{2}$ with probability arbitrarily close to 1 (Notice that the profit of the gambler is $2\cdot Reward - Invest$ because the casino needs to return his stack when he wins). Although we cannot bound $\mathbb{E}\left( \frac{Reward}{Invest}\right)$ even when $p$ is small, we can prove that $\frac{\mathbb{E}[Reward]}{\mathbb{E}[Invest]} \leq p$. 

Suppose a player is investing money into a lottery. At each timestep $t$, the player first commits his investment $c(t)$, then the lottery generate a random variable $X_t$ from some distribution $P_t$. If $X_t \in R$, the player receives a reward of $c(t)$. We use $x_t$ to denote a possible outcome of $X_t$. Assume the player's investment $c(t)$ is a function of the previous outcomes, i.e., $c(t) = f(x_{1:t-1})$. Assume the distribution $P_t$ satisfies that
$$P(X_t \in R \mid X_{1:t-1} = x_{1:t-1}) \leq p, \forall x_{1:t-1}.$$
We must have
$$\mathbb{E}[Reward] \leq p\mathbb{E}[Invest].$$
\begin{proof}
We can express the expected total investment by
\begin{equation}\label{gentle_start:e1}
    \mathbb{E}[Invest] = \sum_{t=1}^\infty \sum_{x_{1:t-1}} P(X_{1:t-1} = x_{1:t-1})f(x_{1:t-1}).
\end{equation}
At the same time, we have
\begin{subequations}\label{gentle_start:e2}
    \begin{align}
    &\mathbb{E}[Reward]\nonumber\\
    ={}& \sum_{t=1}^\infty \sum_{x_{1:t}} P(X_{1:t} = x_{1:t}\text{ and }X_t \in R) f(x_{1:t-1})\label{gentle_start:e2:s1}\\
    ={}& \sum_{t=1}^\infty \sum_{x_{1:t-1}} P(X_{1:t-1} = x_{1:t-1})\nonumber\\
    &\cdot P(X_t \in R \mid X_{1:t-1} = x_{1:t-1})\cdot f(x_{1:t-1})\label{gentle_start:e2:s2}\\
    \leq{}& p\sum_{t=1}^\infty \sum_{x_{1:t-1}}P(X_{1:t-1} = x_{1:t-1})f(x_{1:t-1}).\label{gentle_start:e2:s3}
    \end{align}
\end{subequations}
\eqref{gentle_start:e2:s1} is summing over all possible outcomes $x_{1:t}$ of $t$ consecutive random variables $X_{1:t}$, and we must have
$$P(X_{1:t} = x_{1:t}\text{ and }X_t \in R) = 0$$
if $x_t \not \in R$. In \eqref{gentle_start:e2:s2}, we use the fact that
\begin{equation*}
    \begin{aligned}
    &\sum_{x_t} P(X_{1:t} = x_{1:t}\text{ and }X_t \in R)\\
    ={}& P(X_t\in R\text{ and }X_{1:t-1} = x_{1:t-1})\\
    ={}& P(X_{1:t-1} = x_{1:t-1})P(X_t \in R \mid X_{1:t-1} = x_{1:t-1}).
    \end{aligned}
\end{equation*}
when $x_{1:t-1}$ are fixed.

In \eqref{gentle_start:e2:s3}, we use the assumption that
$$P(X_t \in R \mid X_{1:t-1} = x_{1:t-1}) \leq p.$$

Combining \eqref{gentle_start:e1} and \eqref{gentle_start:e2} gives the conclusion.
\end{proof}











\begin{comment}
\begin{equation}
    \begin{aligned}
    \mathbb{E} \sum_{i} c(x_i)&\leq \sum_{t = 1}^T P(t \in R \mid \cdot \leq t - W) c(t)\\
    &\leq \frac{2}{W}\sum_{t=1}^T c(t).
    \end{aligned}
\end{equation}

\yiheng{Is this correct? Actually we cannot bound the expectation of the ratio between $cost(ALG)$ and $\sum_{t=1}^T c(t)$. For example, consider a company that invests as follows: Let $c(0) = c(1) = \cdots = c(w - 1) = 0$. Set a flag $f = 0$. At timestep $t$:
\begin{enumerate}
    \item If $f = 1$ or $W \not \mid t$, set $c(t + W) = 0$;
    \item Else, suppose $t = kW$. If the player stops at $t$, set $c(t + W) = 0$ and $f = 1$; Else, set $c(t + W) = 2^{k}$.
\end{enumerate}
Then the expected reward is lower bounded by $\frac{\eta}{2}\sum_{t=1}^T c(t)$!
Can we save this by setting an upper bound $S$ on the total amount of the investment and try to derive:$\mathbb{E} \sum_{i} c(x_i) \leq \frac{2S}{W}?$}

Suppose we are on an axis and start from $0$. Our destination is at $T$. Due to a limitation on the amount of the fuel we can take with our vehicle (or aircraft), we have to divide the whole journey into several short trips. Suppose the longest distance we can move at a single step is $L$. Assume there are gas stations (or airports) at every integer points where we can stop by and refuel. However, stopping at each station incurs a different amount of cost, and this cost will be revealed to us when we are $W$ away from the station. (Recall the SOCO prediction window.) For simplicity, we consider the case where $W = L$. In some real situations, $W$ can be much larger or smaller than $L$.

Formally, the game is played as following: 
\begin{enumerate}
    \item \textbf{At the beginning:} Initialize stop point sequence $R = \{x_0\}$, where $x_0 = 0$. The adversary propose nonnegative costs $c(0), c(1), \cdots, c(W - 1)$;
    \item \textbf{When the player arrives at or pass by location $t$:} The adversary propose a nonnegative cost $c(t + W)$ if $t + W \leq T$. Suppose $x_i$ is the last element in sequence $R$. If $t = x_i$, the player commits the next stop point $x_{i+1}$ subject to $x_i + 1\leq x_{i+1} \leq x_i + W$ and $x_{i+1}\in \mathbb{Z}$. $x_{i+1}$ is added into sequence $R$ and revealed to the adversary.
\end{enumerate}

For information, we assume the player does not have any knowledge about the costs during the whole game.

In order to quantify the performance of an online algorithm, we compare the expected cost incurred by the algorithm $\mathbb{E} \sum_i c(x_i)$ with the sum of all costs $\sum_{t = 1}^T c(t)$.\yiheng{Maybe we need to fix this sum.}
\end{comment}

==> prediction.tex <==

\section{Motivation}
While it is straight forward to see that Convex Body Chasing (CBC) is a special case of SOCO by letting the hitting cost function $f_t$ be the indicator function of body $K_t$, it is non-trivial to give a reduction from SOCO to CBC. Theorem \ref{thm:Reduce_SOCO_to_CBC} shows that if we can solve the CBC problem in $(d+1)-$dimension space, we can also solve the SOCO problem in $d-$dimension space with the same movement cost.
\begin{theorem}\label{thm:Reduce_SOCO_to_CBC}
Consider the $d-$dimension SOCO problem where the movement cost function is given by $c(x_t, x_{t-1}) = \norm{x_t - x_{t-1}}_p$. Suppose we have a $C$-competitive algorithm $A$ for $(d + 1)-$dimension CBC problem with the same movement cost function $c(x_t, x_{t-1})$. There exists an $4C$-competitive algorithm $A'$ for $d-$dimension SOCO problem with the movement cost function $c(x_t, x_{t-1})$.
\end{theorem}

A number of works leverage the power of prediction window to achieve a better competitive ratio for SOCO problems (see \cite{lin2012online}, \cite{li2018online}). Since Theorem \ref{thm:Reduce_SOCO_to_CBC} suggests that CBC is equivalent to the most general SOCO problem to some extent, it will be great if we can use prediction window to improve the competitive ratio of CBC.

\begin{definition}[Use prediction efficiently]\label{def:efficient_pred}
We say a SOCO algorithm $ALG$ for a problem setting $P$ can leverage the prediction window efficiently if there exists a function $g: \mathbb{R}^+ \to \mathbb{R}^+$ which is independent with the number of total timesteps $T$, such that $\forall \epsilon > 0$, $\forall W \geq g(\epsilon)$, $ALG$ with a prediction window of length $W$ has a competitive ratio of at most $(1 + \epsilon)$.
\end{definition}

\section{Prediction does not help}
However, Theorem \ref{thm:Pred_not_help} suggests that leveraging the prediction window efficiently (see Definition \ref{def:efficient_pred}) is not possible for general SOCO. A counterexample is Convex Body Chasing.

\begin{theorem}\label{thm:Pred_not_help}
Consider the CBC problem where the movement cost function is given by $c(x_t, x_{t-1}) = \norm{x_t - x_{t-1}}$, where $\norm{\cdot}$ is some genral norm. Suppose an algorithm A can leverage a prediction window of length $w$ and achieve a competitive ratio of $f(d, w)$. There exists an algorithm $A'$ which does not need prediction (i.e. $w = 1$) but also have a competitive ratio of $f(d, w)$.
\end{theorem}

Since any algorithm cannot have a competitive ratio less than $\Omega(\sqrt{d})$ for linear $\ell_2$ movement cost (see \cite{chen2018smoothed}), Theorem \ref{thm:Pred_not_help} suggests that, if the size of the prediction window is finite, the competitive ratio of CBC is always lower bounded by $\sqrt{d}$ as $T \to \infty$.

Another limitation of the CBC problem setting is the constraints on the movement cost function. It has been widely noticed (see \cite{bubeck2019improved}) that when the movement cost function is given by $c_t(x_t, x_{t-1}) = \frac{1}{2}\norm{x_t - x_{t-1}}_2^2$ as in SOCO problems studied in \cite{goel2019beyond}, \cite{goel2018smoothed}, \cite{li2018online}, the competitive ratio can be unbounded. We make this statement formally in Theorem \ref{thm:quad_CBC_impossible}.

\begin{theorem}\label{thm:quad_CBC_impossible}
Consider the CBC problem where the movement cost function is given by $c(x_t, x_{t-1}) = \frac{1}{2}\norm{x_t - x_{t-1}}_2^2$. Provided with a prediction window with length $W$, no algorithm can have a competitive ratio smaller than $T/W$.
\end{theorem}

The negative results in Theorem \ref{thm:Pred_not_help} and Theorem \ref{thm:quad_CBC_impossible} inspire us to add more constraints to the hitting cost functions in SOCO to leverage the power of prediction.

\section{The Limit of Predictions}
In this section, we first propose a new deterministic algorithm, Averaged Regularized Fixed Horizon Control (ARFHC), which can use the prediction window efficiently under a very general set of conditions. It is similar with the Averaged Fixed Horizontal Control proposed in \cite{lin2012online}.

In order to get rid of the convexity condition on hitting cost functions, we then propose Random Regularized Fixed Horizont Control (RRFHC), which is a randomized variation of ARFHC. Although Theorem 2.1 in \cite{bansal20152} shows that randomization does not help in SOCO, it remains unknown whether randomization helps for non-convex hitting cost functions.

Regularized Fixed Horizon Control in phase $h$, $RFHC(h)$, outputs the solution of
\begin{equation}
    \begin{aligned}
    &\min_x \sum_{t=1}^T f_t(x_t) + c(x_t, x_{t-1})\\
    &\text{Subject to }x_t = v_t, \forall t \in \Omega_h,
    \end{aligned}
\end{equation}
where we define $\Omega_h = \{k \mid k \equiv h \mod W, 1 \leq k \leq T\}.$ Notice that $RFHC(h)$ is an online algorithm with a prediction window of length $W$. It can be easily verified that $RFHC(h)$ is an online algorithm that leverages a prediction window of length $W$.

At timestep $\tau \in \Omega_h$, Averaging RFHC (ARFHC) use $RFHC(h)$ to determine the provisioning $x_{\tau + 1}^{(k)}, \cdots, x_{\tau + W}^{(k)}$, and then set $x_{ARFHC, \tau} = \sum_{n=1}^W x_\tau^{(n)}/W$.

The competitive ratio of ARFHC and its decay rate with the length of prediction window is given in Theorem \ref{thm:ARFHC_general_cr_1}. There are two assumptions made in this theorem: the first says the movement cost satisfies some general triangle inequality; the second says, when the point we pick leaves the minimizer of the hitting cost, the hitting cost value grows at least linear in movement cost value.

\begin{theorem}\label{thm:ARFHC_general_cr_1}
Consider the SOCO problem where the movement cost is given by $c(x_t, x_{t-1})$ which satisfies
$$\forall x, y, z, c(x, z) \leq \eta \left( c(x, y) + c(y, z)\right),$$
and the hitting cost function $f_t$ is convex and satisfies
$$\forall x, f_t(x) \geq \lambda \left( c(x, v_t) + c(v_t, x) \right),$$
where $v_t$ is the global minimum of $f_t$. Regularized AFHC has a competitive ratio of $\left( 1 + \frac{1}{W}\max\left(\frac{\eta}{\lambda}, 2(\eta - 1) \right)\right)$ when it has a prediction window of size $W \geq 2$.
\end{theorem}

To show the generality, we show that a series of SOCO works can fit in this problem setting:
\begin{enumerate}
    \item Linear $\alpha-$polyhedral setting (see \cite{chen2018smoothed}), $c(x, y) = \norm{x - y}$, we can pick $\eta = 1$ and $\lambda = \frac{\alpha}{2}$.
    \item Quadratic $m-$Strongly Convex setting (see \cite{goel2018smoothed, goel2019beyond}), $c(x, y) = \frac{1}{2}\norm{x - y}_2^2$, we can pick $\eta = 2, \lambda = \frac{m}{2}$.
    \item Geographical Load Balancing (see \cite{lin2012online}), $c(x, y) = (x - y)^+$, we can pick $\eta = 1$ and $\lambda = \frac{e}{4}$, where $e$ is the minimum cost of running a server. The proof is provided in Appendix \ref{Appendix:Geo}.
\end{enumerate}

Notice that in the last step of the proof of Theorem \ref{thm:ARFHC_general_cr_1}, we use Jensen Inequality, which requires function $cost: \mathbb{R}^{d\times T} \to \mathbb{R}^+ \bigcup \{0\}$ to be convex. The total cost function $cost$ is convex when every $f_t$ is convex. However, we haven't use the convexity of $f_t$ throughout the proof except this step. Therefore, in order to avoid the convexity assumption on hitting costs, we can just picked the phase of RFHC randomly.

\subsection{Deterministic Method}
\input{deterministic_pred.tex}
\subsection{Randomized Method}
\input{randomized_pred.tex}

\input{Underlying_problem.tex}
